Contextual Latent-Movements Off-Policy Optimization for Robotic Manipulation Skills

Parameterized movement primitives have been extensively used for imitation learning of robotic tasks. However, the high-dimensionality of the parameter space hinders the improvement of such primitives in the reinforcement learning (RL) setting, especially for learning with physical robots. In this paper we propose a novel view on handling the demonstrated trajectories for acquiring low-dimensional, non-linear latent dynamics, using mixtures of probabilistic principal component analyzers (MPPCA) on the movements' parameter space. Moreover, we introduce a new contextual off-policy RL algorithm, named LAtent-Movements Policy Optimization (LAMPO). LAMPO can provide gradient estimates from previous experience using self-normalized importance sampling, hence, making full use of samples collected in previous learning iterations. These advantages combined provide a complete framework for sample-efficient off-policy optimization of movement primitives for robot learning of high-dimensional manipulation skills. Our experimental results conducted both in simulation and on a real robot show that LAMPO provides sample-efficient policies against common approaches in literature.

==> legend1.tex <==
\begin{tikzpicture}


\definecolor{color0}{rgb}{0.75,0.75,0}
\definecolor{color1}{rgb}{1,0.25,0}

\begin{axis}[
height=2cm,
width=8cm,
hide axis,
xmin=10,
xmax=50,
ymin=0,
ymax=0.5,
legend columns=-1,
legend entries={{Demonstrations},{Demonstrations (mean)},{LAMPO (samples)}, {LAMPO (mean)}},
legend style={at={(1.0,0.1)}, anchor=north, draw=none, font=\scriptsize, column sep=1ex, line width=2 pt},
]


\addlegendimage{only marks, mark=*color1}
\addlegendimage{no markers, color1}
\addlegendimage{only marks, mark=*, color0}
\addlegendimage{no markers, color0}

\end{axis}

\end{tikzpicture}

==> sections/ablation.tex <==
%\subsubsection{Ablation study}
% Here, we ablate the performance of LAMPO over different algorithmic decision choices. Particularly, we argue over the effect of increasing complexity in the dataset, i.e. the effect if different clusters of movements as in the  \texttt{2d-reacher}. Second, we evaluate the effect of the sample size 

% \subsubsection{Response to Nonlinearities} In the first part of this experiment, we tested our algorithm on the already-mentioned \texttt{2d-reacher}, setting a different number of goal-cluster (from 1 to 4). Clearly, the situation with four cluster is more difficult to solve, as incorporates some non-linear dependencies between the movements, which need to be solved via imitation learning and subsequent policy improvement. 
% In Figure~\ref{fig:nonlinear} we can see the behavior of the imitation learning of CT and LAMPO under the presence of different number of clusterw (where we adapt $K$ to match the number of real clusters). Our algorithm maintains a good behavior across the four different modalities. Furthermore, very interestingly, when we augment the dimension of the latent variable, the performance slightly degrades, showing a higher efficiency with a low dimensional latent representation. CT, instead, struggles at the presence of non-linearities, and solves the imitation learning only with the presence of a single cluster. The reason is that, by performing the linear dimensionality reduction, it looses the information about the non-linear region, and is not able to recover it in the GMM.


% The response in terms of policy improvement is instead observable in Figure~\ref{fig:nonlinearrl} where we test CT and LAMPO with different number of nonlinear regions, and we observe that, while LAMPO manages to learn and improve in all the settings, CT has a drop in performance of several order of magnitude at the presence of different clusters.


% \begin{figure}
% 	\input{figures/ablation2.tex}
% 	\caption{\label{fig:samplesize} \texttt{target-reacher}: (a) While keeping the number of samples per iteration fixed to $500$, we use different number of demonstrations. (b) While keeping the number of demonstration fixed to $1000$, we use different amount of samples per policy improvement. }
% \end{figure}


==> sections/related_work.tex <==
\noindent \textbf{Learning from Demonstration} is an emblematic paradigm for enabling robots to autonomously acquire new skills \cite{atkeson1997robot}.The most prominent methods in robot learning require the mapping of a set of demonstrated motions to a parametric model that represents dynamical systems with complex behaviors \cite{calinon2007learning, ijspeert2013dynamical}. Such models are generally called MPs.
 Dynamic MPs (DMPs) have been thoroughly explored as a robot control policy, as they are stable and robust, however, they lack generalization properties \cite{ude2010task}. ProMPs \cite{paraschos_probabilistic_2013}, on the other hand, is a flexible probabilistic parametric model, which represents movements as distributions over trajectories, and allows the use of probabilistic operations, like conditioning. ProMPs are able to represent complex non-linear dynamical systems, delivering impressive results in acquiring robot skills, like robot hockey \cite{paraschos_using_2018}.		

\noindent \textbf{Dimensionality reduction.}
Applying RL to robots is challenging due to  the high-dimensional continuous spaces. A common practice is to use demonstrations to properly initialize the control policy. Even with good initialization, the performance is not optimal. Hence, researchers have opted for finding sufficient state representations, introducing DR techniques, to encode the latent features present in data \cite{bitzer2010using}. In this line of research, Colom\'{e} et al. \cite{colome_dimensionality_2014} have introduced a probabilistic DR technique of ProMPs in the joint space, using expectation-maximization (EM) over the context variables, for representing the movements in a linear low-dimensional subspace  of the full configuration space. Then, the policy is further optimized via relative entropy policy search (REPS) \cite{peters2010relative}. In \cite{colome_dimensionality_2014-1}, the authors introduced a DR technique of the exploration parameters of DMPs when using a path integral policy improvement algorithm \cite{theodorou2010reinforcement}. In \cite{rueckert_extracting_2015} a low  dimensional latent variable model for ProMPs is extracted using fully Bayesian hierarchical models, which is used only for imitation learning. 
Autoencoded DMPs are proposed in \cite{chen_efficient_2015}, which uses deep autoencoders to find a latent representation
of the movement from the robot's task space, towards generalizing the performance of the DMPs. In \cite{chen_dynamic_2016} the authors proposed the use of a time-dependent variational autoencoder to address the generalization challenges. Dermy et al. \cite{dermy2018prediction} used auto-encoders with ProMPs for efficient human motion prediction.
Colom\'{e} et al. \cite{colome_dimensionality_2018} have proposed a linear DR in the joint space for learning DMPs, however, in \cite{colome_dimensionality_2018-1}, the authors proposed a reduction of the parametric space, as more appropriate for learning MPs. In \cite{delgado2020sample} the authors use parametric DR to learn a mapping from the MPs latent space to a reward for policy improvement. 

\noindent \textbf{Contextual Policy Optimization.} Policies acquired through IL are usually optimized in a RL setting, where the objective lies in acquiring the policy parameters for which we acquire the maximum return \cite{kang2018policy}. Often the policy is warm-started by the demonstrated samples, which is further improved through policy iteration \cite{cheng2018fast}, or the demonstrated and the on-policy samples are mixed \cite{balakrishna2020policy}. However, the importance of generalizing skills led to the introduction of contextual RL methods \cite{klink2020self}. Indeed, contextual policy search has proven to be a data-efficient method for generalizing robot skills over contexts that represent either objectives of
the robot or physical properties of the environment \cite{kupcsik_data-efficient_2013,abdolmaleki2015contextual}. The most relevant line of research to ours is \cite{colome_dimensionality_2018-1}, which uses contextual REPS for optimizing the policy acquired over demonstrations. 

\color{red}
\noindent \textbf{Off-policy methods.}
Off-policy evaluation and improvement are core problem in RL. The off-policy estimation is in fact hard to obtain, due to distribution mismatch \cite{thomas2016data}. \cite{shelton_policy_2001} first introduced the usage of importance sampling to obtain off-policy policy gradient improvement. Recent model-free deep RL methods employ off-policy estimation \cite{haarnoja2018soft}; though, such methods require a vast amount of interactions of the agents with the environment. Notably, our method combines off-policy estimation together with trust-region regularization that contains the estimation variance \cite{peters_relative_2010,schulman_trust_2015, schulman2017proximal}.

%To contain the estimation variance, in many recent works the importance sampling is coupled with a trust region method [REPS, TRPO, PPO, SAC(?)]. Our method, similarly, combines both self-normalized importance sampling and kl-regularization to obtain a robust estimator.}
\color{black}
We propose a novel view on handling the demonstrated trajectories for acquiring lower-dimensional, non-linear latent dynamics, which can later on be optimized by LAMPO, a novel contextual policy gradient algorithm. Contrary to works in literature, our method contributes two important aspects in combining imitation learning with policy optimization. (1) Our proposed MPPCA DR technique allows us to learn a reduced latent representation of the movements over parameters and contexts, preserving their non-linear dependencies. (2) The new contextual off-policy RL algorithm can provide gradient estimates using self-normalized importance sampling \color{red} over the latent space of movements \color{black} from previous experience, hence, making full use of the samples collected through different learning iterations. 
These advantages combined provide a framework for sample-efficient and safe off-policy optimization of MPs for robot learning of complex manipulation skills.

==> sections/virtual.tex <==
\subsubsection{Additional virtual tests}

